GNNerator: A Hardware/Software Framework for Accelerating Graph Neural Networks

Graph Neural Networks (GNNs) use a fully-connected layer to extract features from the nodes of a graph and aggregate these features using message passing between nodes, combining two distinct computational patterns: dense, regular computations and sparse, irregular computations. To address this challenge, we propose GNNerator, an accelerator with heterogeneous compute engines optimized for these two patterns. Further, GNNerator implements feature-blocking, a novel GNN dataflow that beneficially trades off irregular memory accesses during aggregation for regular memory accesses during feature extraction. We show GNNerator achieves speedups of 5.7-37x over an NVIDIA RTX 2080-Ti, and 2.3x-3.8x over HyGCN, a state-of-the-art GNN accelerator.

==> behavior.tex <==
\putsec{GNN Accelerator Motivation}{motivation}
In this section, we describe the computational characteristics of graph neural networks that drive the design of a GNN accelerator.

\noindent\textbf{Feature Extraction Stage.} The feature extraction stage is usually implemented as a fully-connected layer, in which a node's feature vector is multiplied by a weight matrix, producing a new feature vector, \emph{i.e.}, a layer is essentially a matrix-vector multiplication. However, in order to allow GNNs to generalize to different sized graphs, GNNs typically share the weight matrix across the vertices (edges), meaning that a batch of feature vectors can be processed together with the same weight matrix, resulting in a matrix-matrix multiplication. Thus, the feature extraction stage is characterized primarily as a dense, regular computation with high data reuse of weights. A compute engine for the feature extraction stage, therefore, should have ample compute, with enough internal bandwidth to feed that compute while taking advantage of the large amount of weight reuse.

\noindent\textbf{Aggregation Stage.} The aggregation stage, by contrast, is a highly sparse, irregular kernel, much like many other graph-processing workloads. However, there is one key difference between the aggregation stage and other graph processing kernels. In traditional graph processing applications, the graph data tends to be quite small, on the order of a few bytes per node or edge. In contrast, within a GNN's aggregation stage, the features communicated across vertices can be much larger, on the order of up to thousands of bytes. The large dimension size of the features compared to traditional graph analytics workloads means that there is ample opportunity for \emph{intra}-node parallelism, as each element within a feature for a given node can be processed in parallel. This is in addition to the \emph{inter}-node parallelism present in both the feature extraction and aggregation stages that results from the large amount of nodes that each need to be updated independently in a GNN layer. 
%Secondly, the large dimension size of the features can actually help to reduce the irregular nature of the aggregation stage as compared to other graph-based workloads, as instead of each vertex needed to load one or two bytes per neighbor, each vertex instead must load many bytes, which can result in better coalesced memory accesses. A compute engine for the aggregation stage, therefore, should exploit both the inter- and intra-node parallelism that results from the longer node features, as well as design the memory system around the wider accesses seen in the aggregation stage as compared to other graph accelerators such as Graphicianado \cite{graphicionado}. 


The feature extraction and aggregation stages exhibit a producer-consumer relationship. Further, one stage need not be completely finished before the other stage can begin. Therefore, there also exists inter-stage (pipeline) parallelism, which can be exploited in a specialized architecture.

%\noindent\textbf{Feature Extraction vs Aggregation Stage.} Above, we describe the unique characteristics of the two different kernels present in GNNs, as well as the specific architectural desiderata that results. However, a crucial question is also the relative importance of the two stages, as this would dictate the amount of resources that should be dedicated to them. 
%
%
%%----------------------------------------------------------------------------------
%\begin{figure}[tb]
%	\centering 
%	\includegraphics[width=\columnwidth]{active_breakdown_full.pdf}
%	\vspace{-3pt}
%	\caption[Breakdown between feature extraction and aggregation]{At lower hidden dimension sizes, the aggregation stages dominate the run time over the feature extraction stages. However, at the large dimension size of 1024, this trend reverse. Feature extraction always dominates the run time for the GraphSage-Max network, due to the additional linear layer present before aggregation}
%    %\vspace{-0.1in} 
%	%\vspace{-0.2in} 
%	\label{fig:dnngnnbreakdown}
%\end{figure}
%%----------------------------------------------------------------------------------
%
%To that end, we investigate the relative breakdown in execution time between the aggregation kernels and the feature extraction kernels running on a GNN accelerator design with comparable performance to HyGCN. In particular, we examine this breakdown as a function of the hidden layer's dimension size. As shown in \figref{fig:dnngnnbreakdown}, the aggregation stages dominate the run time for smaller dimension sizes. This is in line with finding from other GNN accelerators, such as \cite{hygcn, engn}. However, at larger, more production-like networks sizes, this trend reverses and the linear layers dominate the run time. Note that the linear layers always dominates the run time for the GraphSage-Max network; this is a result of the additional linear feature extractor present in the  pooling stage. This implies that the needs of the two stages must be carefully balanced, as the bottleneck in GNN processing on a custom architecture depends on the size of the network; smaller networks are bottlenecked by graph processing, whereas larger networks are bottlenecked by fully connected, dense layers.
%
%%
%%%----------------------------------------------------------------------------------
%%\begin{figure*}[h]
%%	\centering 
%%	\includegraphics[width=\textwidth]{forward_visualization}
%%	\caption{Forward pass of one graph network block in a PinSage network, applied to a sample graph with four nodes (a). For clarity, we focus only on node A. To compute the updated edge features as in line 11, \textit{z'}, each edge's source node feature \textit{h} is passed through a fully-connected layer (b). Note that the nodes are not concatenated, but rather are analogous to different samples in a minibatch. Next, each node \textit{aggregates} information from its \textit{incoming} edges using a symmetric function such as max to obtain an aggregated feature vector $\bar{z}'$ (c) as in line 12. Finally, (d) the aggregated feature and the original node feature are combined and passed through another linear layer to obtain an updated node feature, $h'$, as in line 13. This process can be repeated for multiple GNN layers.}
%%    \vspace{-0.1in} 
%%	\label{fig:forward}
%%\end{figure*}
%%%------------
%%
%%
%%\putsubsec{GNN Execution}{gnn_execution}

In summary, a GNN accelerator should be designed with following characteristics in mind. First, in order to efficiently compute the feature extraction stage, the architecture should contain a large compute array for performing matrix-matrix multiplications, optimized for a large amount of weight reuse. Second, the graph engine should be optimized for both the abundant inter- and intra-node parallelism present in GNNs. Finally, there must be fine-grained control between the two compute engines in order to allow for inter-stage parallelism. 


==> old_background.tex <==
\putsec{Background}{old_background}
Graph neural networks (GNNs) have attracted significant interest in the machine learning community, but have not yet been explored in detail by computing system designers. In this section, we will provide a brief introduction into GNNs. A more complete introduction can be found in recent survey papers \cite{survey2019, review2018}.

\putsubsec{Graph Definition and Representation}{graphs}
A graph $G$ is a data structure defined by two unordered sets: its vertices, $V$, and the edges, $E$, between those vertices. We will denote the $i$-th node as $\mathbf{v}_i$. The directed edge between nodes $i$ and $j$ is defined as $\mathbf{e}_{i,j}$, where \textit{i} is the source node and \textit{j} is the destination. Further, each node and edge may have one or more features associated with them, referred to as $\mathbf{h}_i$ and $\mathbf{h}_{i,j}$, respectively. Finally, a graph may also have one or more global features, $\mathbf{u}$, associated with the entire graph.

Graphs can be stored either using an adjacency matrix or adjacency list representation. In an adjacency matrix representation, the adjacency matrix, $\mathbf{A}$, stores \todo{matrix explanation}. This results in a large amount of wasted storage space, as the graphs tend to be very sparse. On the other hand, this representation allows for the use of highly optimized sparse kernels.

In an adjacency list representation, \todo{adjacency list explanation}. Compressed sparse row (CSR) and compressed sparse column (CSC) are two popular formats for adjacency list representation. The main advantage of this representation is that it saves memory space; however, it also results in many random data accesses.

\putsubsec{Edge Dataflows}{eflows}
Stuff.

\putsubsec{Graph Sharding}{sharding}
Many real-world graphs are too large to fit into any given level of the memory hierarchy (last-level cache, main memory, etc). This severely degrades performance of graph processing algorithms, as it makes it extremely difficult to exploit the limited spatial locality available. To address this, graphs are often broken into smaller pieces, such that each subgraph can fit in the given level of memory, in a process referred to as \emph{graph sharding} \cite{graphchi, nxgraph, gridgraph}. Similar to \cite{gridgraph}, we adopt a two-dimensional sharding paradigm, as depicted in \figref{fig:shard_visual}. In this paradigm, a graph's edge list is divided in shards such that each shard contains a maximum of $n^2$ edges. A shard is then referred to by the tuple $(U, V)$, such that shard $(U, V)$ contains the edges whose source nodes are in the set $[U*n, (U+1)*n)$ and whose destination nodes are in the set $[V*n, (V+1)*n)$.

\begin{figure}[h]
	\centering 
	\includegraphics[width=\columnwidth]{shard_visual.png}
	\caption{Visualization of a two-dimensional graph sharding algorithm that divides an edge list into shards such that Shard $(U, V)$ is the set of all edges such that $e.u \in [U*n, (U+1)*n)$ and $e.v \in [V*n, (V+1)*n)$. The resulting subgraphs can then be processed in either a source-stationary (dotted arrow) or destination-stationary (slanted arrow) manner.}
	\label{fig:shard_visual}
\end{figure}

\putsubsec{Graph Neural Networks}{gnns}
Graph neural networks are a widely diverse family of networks. Throughout this paper, we adopt the definition provided by DeepMind \cite{graphnetworks}, shown in Equation \eqref{eq:graphnetwork}, which generalizes a large number of popular GNNs \cite{pinsage, mpgnn, gatedgnn, gat, struct2vec}. Under this formulation, there are three main stages to a generalized GNN layer: edge update, node update, and global update.

\noindent\textbf{Edge update.} In the edge update stage (lines 2-4), an update function, $\phi^e$, is mapped to every edge in $E$. This function updates an edge's features based on the edge's current feature, the source node's current feature, the destination node's current feature, and a global feature. A single fully-connected layer is often used as the update function, though other functions may be used.

\noindent\textbf{Node update.} In the node update stage (lines 5-9), the updated edge features are first aggregated on a per-node basis according to some aggregation function $\rho^{e->v}$. After the edge features are aggregated, an update function, $\phi^v$, is mapped to every node in $V$. This function updates a node's features based on the aggregated edge feature, the current node feature, and a global feature. Again, a single fully-connected layer is often used as the update function.

\noindent\textbf{Global update.} In the global update stage (lines 10-15), the updated edge features and node features are both aggregated on a global basis. Note that this in contrast to the previous edge aggregation, which was performed per-node. As above, the global feature is then updated using an update function, $\phi^u$, that is based on the aggregated edges and nodes.

These three stages make up a single, generalized GNN layer. A fully GNN can be constructed by stacking these layers. By stacking layers, a GNN can incorporate information from nodes that are increasingly far away from the original node. For example, a single layer GNN only considers a node's neighbors, while a two layer GNN will consider nodes in the two-hop neighborhood. Notice, however, that this results in an exponential increase as the depth increase. In order to mitigate the overhead introduced by this exponential increase, GNNs designed for extremely large graphs, such as those used in web recommendation systems, introduce an initial preprocessing stage: subgraph sampling \cite{pinsage, fastgcn, cluster-gcn, vr-gcn}.

\noindent\textbf{Subgraph sampling.} In subgraph sampling (lines 2-7), a subgraph is sampled from a much larger graph. The method of sampling is of ongoing research, but common techniques include various random walks and clustering algorithms. The subgraphs are constructed such that the number of nodes in a given neighborhood will be constrained even as the depth of the GNN increases. Once a subgraph is sampled, the desired GNN is then executed using the subgraph as input.

A specific GNN can be realized from this specific framework by specifying the exact form of the aggregation and update functions. These functions can also ignore subsets of the inputs. For example, lines 11, 12, and 13 in Equation \eqref{eq:pinsage} correspond to lines 2, 5, and 6 in Equation \eqref{eq:graphnetwork}, respectively. In this example, there are no global attributes. For a complete discussion on how specific GNNs can be specified, please see \cite{graphnetworks}.

%----------------------------------------------------------------------------------
%\begin{figure*}[h]
%	\centering 
%	\includegraphics[width=\textwidth]{gnn_block}
%	\caption{Generalized Graph Neural Network \todo{Update this in latex}}
%    \vspace{-0.1in} 
%	\label{fig:gnn_block}
%\end{figure*}
%------------

%-----------------------------------------------------
\SetKwInput{Input}{Input}
\SetKwInput{Output}{Output}
\SetKw{Let}{Let}
\begin{algorithm}
\caption{Steps of a Graph Network block}
\label{eq:graphnetwork}
\Input{Graph $(V,E)$; node attributes $h$, edge attributes $z$, global attributes $g$}
\Output{Updated node attribute $h'$; updated edge attributes $z'$, updated global attributes $g'$}
\For{$e \in E$}{
    \tcc{Compute updated edge attributes}
    $\mathbf{z}_e' \gets \phi^e(\mathbf{z}_e, \mathbf{h}_{e.u}, \mathbf{h}_{e.v}, \mathbf{g})$
}
\For{$u \in V$}{
    \Let $E_v' = \{(\mathbf{z}_{(u, v)}', \mathbf{h}_u, \mathbf{h}_v)| v \in N(u)\}$\\
    \tcc{Aggregate edge attributes per node}
    $\bar{\mathbf{z}_u}' \gets \rho^{(e \to v)}(E_v')$\\
    \tcc{Compute updated node attributes}
    $\mathbf{h}_u' \gets \phi^v(\mathbf{h}_u, \bar{\mathbf{z}_u}', \mathbf{g})$
}
\tcc{Aggregate edge attributes globally}
$\bar{\mathbf{z}} \gets \rho^{(e \to g)}(E')$\\
\tcc{Aggregate node attributes globally}
$\bar{\mathbf{h}} \gets \rho^{(e \to g)}(V')$\\
\tcc{Compute updated global attribute}
$\mathbf{g}' \gets \phi^g(\bar{\mathbf{z}}, \bar{\mathbf{h}}, \mathbf{g})$
\end{algorithm}

%-----------------------------------------------------
\begin{algorithm}
\caption{PinSage algorithm}
\label{pinsage}
\Input{Graph $G$; number of layers $L$; neighborhood function $N : V \rightarrow 2^V$; symmetric aggregation function $\gamma$}
\Output{Embeddings $\mathbf{z}_u, \forall u \in V$}
\For{$i \gets 0$ \KwTo $NumMiniBatches$}{
    \tcc{Generate subgraphs}
    $M = RANDOMSUBSET(V)$ \\
    $S^{(L)} \leftarrow M$ \\
    \For{$l \gets L$ \KwTo  $0$}{
        $S^{(l-1)} \gets S^{(l)} $\\
        \For{$u \in S^{(l)}$}{
            $S^{l-1} \gets S^{k-1} \cup N(u)$
        }
    }
    \tcc{Perform graph network block}
    $\mathbf{h}_u^{(0)} \gets \mathbf{x}_u, \forall u \in S^{(0)}$\\
    \For{$l \gets 1$ \KwTo $L$}{
        \For{$u \in S^{(l)}$}{
            $\mathbf{z}' \gets \{ReLU(\mathbf{Q}\mathbf{h}_v + \mathbf{q}) | v \in N(u)\}$\\
            $\bar{\mathbf{z}_u} \gets \gamma(\mathbf{z}')$\\
            $\mathbf{h}_u \gets ReLU(\mathbf{W} \cdot CONCAT(\mathbf{h}_u, \bar{\mathbf{z}_u}) + \mathbf{w})$\\
        }
    }
    \tcc{Generate final embeddings}
    \For{$u \in M$}{
        $\mathbf{z}_u \gets \mathbf{G}_2 \cdot ReLU(\mathbf{G}_1\mathbf{h}_u^{(L)} + \mathbf{g})$
    }
}
\end{algorithm}
%-----------------------------------------------------



==> overview.tex <==
\putsec{GNNerator Overview}{old_overview}
\framework{} is a framework for quickly evaluating the high-level hardware/software co-design of graph neural network accelerators. It consists of \accel{}, a functional- and performance-level  graph neural network accelerator generator capable of simulating many different hyperparameters, a well-defined computation model, and a software framework for mapping graph neural networks to \accel{} using the computational model.  
%----------------------------------------------------------------------------------
\begin{figure}[h]
	\centering 
	\includegraphics[width=\columnwidth]{methodology}
	\caption{Todo}
    \vspace{-0.1in} 
	\label{fig:methodology}
\end{figure}
%------------
In the framework, a given GNN is first transformed into a \accel{} intermediate representation. This IR, along with the graph(s) to be used in inference and a configuration file specifying the desired \accel{} hardware and software parameters, are then compiled into a binary and pre-processed graph. The \accel{} simulator then ingests these inputs, and produces both a functional output, which can be compared to a golden model running on a commodity platform, as well an estimate of the performance and power of the architecture candidate.

\todo{TABLEREF} shows the various hardware and software knobs that are exposed to the system designer in \framework{}. Using these combination of hyperparameters, \framework{} can be used to inform both high-level architectural decisions, such as how much compute should be dedicated to the feature extraction stage \emph{vs.} the feature aggregation stage, as well as high-level software decisions, such as how to efficiently compute a given sharded graph. %Since \framework{} is a functional simulator as well, it can be used to investigate the network-level impacts as well, such the impact of eliminating atomic locks or of quantization.

%\begin{table*}[]
%\centering
%\begin{tabular}{ccc}
%\hline
%\multicolumn{3}{c}{Hardware Hyperparameters}                                              \\ \hline
%Input Feature SRAM Size & Edge SRAM Size               & Modified Feature SRAM Size       \\
%On-chip Memory Latency  & DRAM Latency                 & DRAM Bandwidth                   \\
%Frequency               & Number of GPEs               & Number of Lanes in GPE           \\
%Number of SFUs          & Latency of Each Compute Unit & Init Rate of Each Compute Unit   \\
%DNN Filter SRAM Size    & DNN Output Map SRAM Size     & DNN Input Map SRAM Size          \\
%Systolic Array Height   & Systolic Array Width         & DNN SRAM Shared                  \\ \hline
%\multicolumn{3}{c}{Software Hyperparameters}                                              \\ \hline
%Edge Dataflow           & DNN Stationality             & \# of Dimensions On-chip/Feature
%\end{tabular}
%\end{table*}

In the following sections, we step through the various components of the \framework{} framework, explaining each one in depth and demonstrating how it is used to model the different hyperparameters outline in \todo{TABLEREF}.

==> software.tex <==
\putsec{Programming GNNerator}{programming-gnn}
To program \gnnaccel{}, we develop a compiler and a runtime environment.
\putsubsec{Compiler}{gnnerator-compiler}
The compiler takes as input a GNNerator program, which can be obtained from a graph neural network framework such as Deep Graph Libary (DGL). This program, consisting of GNNerator ISA pneumonics as well as pseudoinstructions indicting off- and on-chip convoys, defines the graph neural network to be executed. A description of the \gnnaccel{} micro-architectural configuration is also provided as an input to the compiler. Using this information, the compiler first shards the graph into small subgraphs to be executed.

%\begin{figure}[h]
%	\centering 
%	\includegraphics[width=\columnwidth]{sharding_algo}
%	\caption{\todo{caption}} 
%	\label{fig:shard_code}
%\end{figure}

%-----------------------------------------------------
\SetKwInput{Input}{Input}
\SetKwInput{Output}{Output}
\SetKw{Let}{Let}
\begin{algorithm}
\caption{Algorithm to determine number of nodes that can be kept on-chip}
\label{eq:shardalgo}
\Input{Graph $G$; \gnnaccel{} configuration $params$; number of input features $ifeat$; number of output features $ofeat$}
\Output{Number of nodes per shard $N_{shard}$}
$N_{shard}^{agg} = params.omembytes / (params.blockD \cdot ofeat)$ \\
$N_{shard}^{inp} = params.imembytes / (params.blockD \cdot ifeat)$ \\
$E_{max} = params.E_{max} $ \\
\tcc{First, try the largest possible $N_{shard}$}
$N_{shard} = min(N_{shard}^{agg}, N_{shard}^{inp}, |G.V|)$ \\
$E_{shard} = COUNT\_EDGES(G, params, N_{shard})$ \\
\If{$E_{shard} < E_{max}$}{
    return $N_{shard}$\\
}
\tcc{Try based on sampled connectivity}
$c = E_{shard} / N_{shard}^2$ \\
$N_{shard} = \sqrt{E_{max}/c}$ \\
$E_{shard} = COUNT\_EDGES(G, params, N_{shard})$ \\
\If{$E_{shard} < E_{max}$}{
    return $N_{shard}$\\
}
\tcc{Default to worst case}
$N_{shard} = \sqrt{E_{max}}$ \\
return $N_{shard}$ \\
\end{algorithm}
%-----------------------------------------------------

This is done by first analyzing the code to determine the maximum number of node features that must be resident on-chip for the given network. In the example code in \figref{fig:code}, this would be one input node feature and one output node feature: \texttt{h\_act} and \texttt{neigh}. The maximum number of node features in turn sets the maximum number of nodes that can be on-chip, as there must be enough memory for each node to have that number of features on-chip.

However, this only ensures that the nodes can fit on-chip, but we must also make sure there is space for the edges as well. To do, we attempt to shard the graph based on that optimistic nodes per shard. When attempting to shard the graph, we determine the maximum number of edges that would be required to support that many nodes per shard. Note that this completely dependent on the graph structure and cannot be determined a priori. If the maximum number of edges required fits on-chip, the graph sharding processes is complete. Otherwise, the maximum number of edges is used to estimate the connectivity of the graph, which is then used to estimate a new number of nodes per shard. We again attempt to shard the graph, determining the maximum number of edges that would be required to support that many nodes per shard. If the edges fit on-chip, we terminate the sharding process. Finally, if the sampled connectivity attempt does not work, we assume a worst case situation, wherein the nodes per shard is set based on assuming that the network is fully connected, thus guaranteeing the graph shards produced will fit on-chip. This process is summarized in Equation~\ref{eq:shardalgo}.

After sharding the graph, the compiler produces the final machine code, using the parameters determine during the graph sharding process to populate the final symbols, \emph{e.g.,} the location in on-chip memory of each of the node features.



%\begin{figure}[h]
%	\centering 
%	\includegraphics[width=\columnwidth]{gsagemax_code}
%	\caption{\todo{caption}} 
%	\label{fig:code}
%\end{figure}


\begin{figure*}[htb]
	\centering 
	\includegraphics[width=\textwidth]{edge_opts}
	\caption[Optimizing edge layouts in \gnnaccel{}]{In this example, the main memory has a width of two edges. (a) Using a naive edge memory layout where the edges are sorted based on the destination node results in idle cycles for GPE1 while GPE0 is being loaded, as well as requires enough space to buffer three edges at once. (b) Using a interwoven memory layout eliminates the idle cycles and reduces the number of edges that must be buffered to only one edge.}
	\label{fig:edge_opt}
\end{figure*}

\putsubsubsec{Edge Layout Optimization}{edgelayout}
As discussed in \secref{sec:gnn-arch}, the \texttt{Shard} \texttt{Edge} \texttt{Fetcher} reads a sharded edge list from main memory and distributes these edges to the private on-chip edge memories of each GPE. In order to realize an efficient "pull"-based ("push"-based) dataflow, all of the edges with the same destination (source) should be consecutive in the on-chip edge memories, as described in \secref{sec:gnn-arch}. However, storing edges naively in a consecutive fashion like that results in inefficient memory transfers. There are two main reasons for this. First, as discussed in \secref{sec:gnn-arch}, each GPE contains an edge memory and edges are distributed to these edge memories such that all edges with the same source (destination) are stored in the same edge memory. If these edges are consecutive in main memory, then usually only one edge memory will be used at a time while the other edge memories are idle, waiting for the set of edges that map to them. Further, even the accesses to the active memory are inefficient. This is because the DRAM width is often much larger than the memory width of the on-chip edge memories, which have a width wide enough to allow one edge access per GPE per cycle. As a result, if all of the edges loaded in a DRAM transaction are destined for the same GPE's on-chip memory, there will be many conflicts, As a result, the architecture would require more on-chip memory, such as queues, to store the stalled DRAM transactions as they are processed. To avoid this, the compiler has an optimization pass after the sharding step, wherein the edges are rearranged in order to pack as many edges from \emph{different} GPEs into a DRAM transaction as possible. This is accomplished by first forming \# GPE different edge lists, where each edge list consists of the edges to be assigned to that GPE. These edge lists are then recombined into a single edge list by storing one edge from each GPE in a round-robin fashion. This results in both more on-chip edge memories being active at one time as well as reducing the required on-chip edge storage, as shown in the visual comparison between the unoptimized and optimized cases in \figref{fig:edge_opt}.

\putsubsubsec{Feature Memory Layout Optimization}{featlayout}
For the same reasons, feature memories should not be laid out sequentially in memory-- that is, it is inefficient to store an entire feature for node 0, followed by the same feature for node 1, and so on. This would again result in only one GPE's on-chip memory being accessed at one time and increase the amount of on-chip storage needed to buffer DRAM transactions. We use a similar round robin strategy to optimize the memory layout, with the additional constraint that the features are divided into chunks of \texttt{\# of Lanes} in order to match the width of the on-chip scratchpads.



